Predictive Display with Perspective Projection of Surroundings in Vehicle Teleoperation to Account Time-delays

Teleoperation provides human operator sophisticated perceptual and cognitive skills into an over the network control loop. It gives hope of addressing some challenges related to vehicular autonomy which is based on artificial intelligence by providing a backup plan. Variable network time delays in data transmission is the major problem in teleoperating a vehicle. On 4G network, variability of these delays is high. Due to this, both video streaming and driving commands encounter variable time delay. This paper presents an approach of providing the human operator a forecast video stream which replicates future perspective of vehicle field of view accounting the delay present in the network. Regarding the image transformation, perspective projection technique is combined with correction given by smith predictor in the control loop. This image transformation accounts current time delay and tries to address both issues, time delays as well as its variability. For experiment sake, only frontward field of view is forecast. Performance is evaluated by performing online vehicle teleoperation on street edge case maneuvers and later comparing the path deviation with and without perspective projection.

==> sections/09-bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{JaiPrakash.png}}]%
{Jai Prakash}
was born in Delhi, India in 1990. He received the B.Tech. degree in Production Engineering from the National institute of technology, Trichy, India in 2012 and M.S. degree in Mechanical Engineering from the Politecnico di Milano, Italy in 2018. From 2018 to 2019, he was a research assistant in Mechanical Engineering Department of Politecnico di Milano. Since 2019, he is a doctoral candidate in Mechanical Engineering Department of Politecnico di Milano. His research interests include computer-vision, robotics, and vehicle dynamics.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{mic.jpg}}]%
{Michele Vignati}
received his M.S. degree (2013) and PhD (2017) in Mechanical Engineering from Politecnico di Milano with thesis on control strategies for distributed powertrain of hybrid and electric vehicles. From 2019 he is Assistant Professor (RTDA) in the research field of applied mechanics. In particular, he focuses on mechanical systems dynamics and control applied in the automotive field of which he has more than 20 publications in international journals and conferences. In 2018 he won the best paper award for a paper presented at the AVEC’18 international conference. He worked on tire dynamics and modelling in cooperation with Pirelli. He works in autonomous driving field and in vehicle modelling, testing, state estimation, and active control systems.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{daniele.png}}]%
{Daniele Vignarca}
is currently a research fellow in mechanical engineering department at Politecnico di Milano. He obtained the M.S. degree in Mechanical Engineering from Politecnico di Milano, Italy, in 2020. His research activity is focused on connected and autonomous vehicles with a focus on V2I communication.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{edo.png}}]%
{Edoardo Sabbioni}
received his PhD in Mechanical Systems Engineering in 2007 and currently works as Associate Professor at the Department of Mechanical Engineering of Politecnico di Milano. His main research activities are in the field of stability, dynamics and control of mechanical systems, with applications to road and rail vehicles. He is also involved in research activities within the fields of aerodynamics and mechatronics. More in particular, he carried out numerical-experimental researches concerned with active safety of vehicles, design of control systems to improve vehicle handling and ride comfort, design of HiL (Hardware-in-the-Loop) test benches, electric and hybrid electric vehicles, autonomous and connected vehicle, “smart” tires technology, cross wind on road/rail vehicles. He is an author of more than 140 scientific publications, most of which published on peer-reviewed journals or presented at international conferences and he is a member of the Editorial Board of Shock and Vibration.

During his research activity, he cooperated and still cooperates with the main Italian automotive/railway industries and he was involved in several Italian and EC funded projects.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{cheli.jpg}}]%
{Federico Cheli}
received the M.S. degree in mechanical
engineering from the Politecnico di Milano, Milano,
Italy, in 1981. He is currently a Full Professor at the
Department of Mechanical Engineering, Politecnico di
Milano and author of more than 380 publications on
international journals and conferences. His scientific
activity concerns research on vehicle performance, handling and comfort problems, active control, ADAS, and
electric and autonomous vehicles. He is a member of
the editorial board of the International Journal of Vehicle Performance and International Journal of Vehicle
Systems Modeling and Testing.
\end{IEEEbiography}
